Deeper Text Understanding for IR with Contextual Neural Language Modeling

Neural networks provide new possibilities to automatically learn complex language patterns and query-document relations. Neural IR models have achieved promising results in learning query-document relevance patterns, but few explorations have been done on understanding the text content of a query or a document. This paper studies leveraging a recently-proposed contextual neural language model, BERT, to provide deeper text understanding for IR. Experimental results demonstrate that the contextual text representations from BERT are more effective than traditional word embeddings. Compared to bag-of-words retrieval models, the contextual language model can better leverage language structures, bringing large improvements on queries written in natural languages. Combining the text understanding ability with search knowledge leads to an enhanced pre-trained BERT model that can benefit related search tasks where training data are limited.

==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

Version 1.36    Bug fixes
		Moved PACMPL to acmlarge format
		New journal: PACMHCI
		Added the possibility to adjust number of author
		boxes per row in conference formats
		
Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
		Added processing of one-compoment ccsdesc nodes
		Bug fixes.
		Made the height a multiple of \baselineskip + \topskip
		Added cleveref
		We no longer print street address in SIGs

Version 1.41    Rearranged bib files
		Added new badges

Version 1.42    Deleted ACM badges
		Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
		Empty DOI and ISBN suppress printing DOI or ISBN lines
		Separated theorem code into acmthm.sty, loaded by default.
		Article number can be set for proceedings.
		New commands: \acmBooktile, \editor.
		Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
		from Overleaf

Version 1.46    Bug fixes for bibliography:  label width is now calculated
		correctly.
		All PACM now use screen option.  This requires etoolbox.
		Added subtitle to ACM reference format.
		Now acmart is compatible with fontspec.
		\thanks is now obsolete.  The addresses are automatically
		added to the journal version;  this can be overriden with
		\authorsaddresses command.
		Deleted the rule at the end of frontmatter for all formats.
		Deleted new line before doi in the reference format.
		Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal:  THRI

Version 1.48    Bug fixes
		Review mode now switches on folios

==> sections/bak-table1.tex <==
 
\begin{table*}[th]
\caption{
Search effectiveness on \textbf{Robust04} and \textbf{ClueWeb09-B}. $\dagger$ indicate statistically significant improvements over \texttt{Coor-Ascent}. \textcolor{red}{remove nDCG@10 for space?}}\label{tab:overall}

\def\arraystretch{0.95}
\vspace{-0.15in}
\setlength\tabcolsep{1.5pt}
\begin{tabular}{l|ccc|ccc||ccc|ccc}
\hline \hline
\multirow{3}{*}{Model} & \multicolumn{6}{c||}{Robust04} & \multicolumn{6}{c}{ClueWeb09-B} \\
 & \multicolumn{3}{c|}{Title Query } & \multicolumn{3}{c||}{Description Query } & \multicolumn{3}{c|}{Title Query } & \multicolumn{3}{c}{Description Query }  \\
                        & nDCG@10   & nDCG@20   & MAP     & nDCG@10      & nDCG@20     & MAP  & nDCG@10   & nDCG@20   & MAP     & nDCG@10      & nDCG@20     & MAP       \\ \hline
LM                     & 0.437     & 0.417     & 0.211   & 0.433        & 0.409       & 0.216
& 0.257 & 0.268 & 0.165 & 0.231 & 0.234 & 0.131 \\
SDM                    & 0.448     & 0.427     & 0.222   & 0.454        & 0.427       & 0.229    & 0.268 & 0.279 & 0.178 & 0.235 & 0.235 & 0.138 \\ \hline
%QE                     & 0.439     & 0.424     & 0.239   & 0.437        & 0.416       & 0.248     & 0.264 & 0.272 & 0.168 & 0.232 & 0.236 & 0.133 \\ \hline
RankSVM                & 0.439     & 0.420     & 0.213   &   0.466  &   0.443      &   0.231 & 0.287 & 0.289 & 0.167 & 0.246 & 0.242 &  0.139 \\
Coor-Ascent            & 0.448     & 0.427     & 0.216   & 0.479       &     0.449        &    0.232       &0.299 & 0.295 & 0.161 & 0.244 & 0.238 & 0.137 \\ \hline
DRMM                   &  0.442    & 0.422     &  0.213  &      0.435        & 0.412    & 0.219           &  0.269 & 0.275 & 0.160 & & & \\ \hline
%K-NRM                  & 0.418           &   0.396        & 0.192     &  0.361            & 0.333           &   0.179      & & & & & &  \\ \hline
%Conv-KNRM-fixemb                  &           &           &         &              &             &         & & & & & &  \\ \hline
BERT-FirstP      & 0.472     & 0.444     & 0.212   & 0.551        & 0.506       & 0.240     & 0.291 & 0.286 & 0.166 & 0.274 & 0.272 & 0.157    \\
BERT-MaxP        & 0.497     & 0.467     & 0.233   & 0.572        & 0.528       & 0.263   & & & & & &  \\ 
BERT-SumP        &      &      &    &         &        &    & & & & & &  \\ 
\hline \hline 
 

\end{tabular}
\end{table*}
